FADE: Few-shot/zero-shot Anomaly Detection Engine using Large Vision-Language Model

Automatic image anomaly detection is important for quality inspection in the manufacturing industry. The usual unsupervised anomaly detection approach is to train a model for each object class using a dataset of normal samples. However, a more realistic problem is zero-/few-shot anomaly detection where zero or only a few normal samples are available. This makes the training of object-specific models challenging. Recently, large foundation vision-language models have shown strong zero-shot performance in various downstream tasks. While these models have learned complex relationships between vision and language, they are not specifically designed for the tasks of anomaly detection. In this paper, we propose the Few-shot/zero-shot Anomaly Detection Engine (FADE) which leverages the vision-language CLIP model and adjusts it for the purpose of industrial anomaly detection. Specifically, we improve language-guided anomaly segmentation 1) by adapting CLIP to extract multi-scale image patch embeddings that are better aligned with language and 2) by automatically generating an ensemble of text prompts related to industrial anomaly detection. 3) We use additional vision-based guidance from the query and reference images to further improve both zero-shot and few-shot anomaly detection. On the MVTec-AD (and VisA) dataset, FADE outperforms other state-of-the-art methods in anomaly segmentation with pixel-AUROC of 89.6% (91.5%) in zero-shot and 95.4% (97.5%) in 1-normal-shot. Code is available at https://github.com/BMVC-FADE/BMVC-FADE.

==> figs/method.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/method_fig.pdf}
    \caption{Different anomaly detection pipelines of FADE. (a) Zero-shot language-guided AC; (b) Zero-shot language-guided AS; (c) Zero-shot vision-guided AS; (d) Few-shot vision-guided AC and AS}
    \label{fig:method}
\end{figure*}


==> figs/prompts.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/prompts_fig.pdf}
    \caption{An instruction given to ChatGPT and its responses.}
    \label{fig:chatgpt_prompts}
\end{figure*}


==> figs/prompts1.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figs/prompts1_fig.pdf}
    \caption{ChatGPT prompt ensemble 1}
    \label{fig:chatgpt_prompts1}
\end{figure*}


==> figs/prompts2.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figs/prompts2_fig.pdf}
    \caption{ChatGPT prompt ensemble 2}
    \label{fig:chatgpt_prompts2}
\end{figure*}


==> figs/prompts3.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figs/prompts3_fig.pdf}
    \caption{ChatGPT prompt ensemble 3}
    \label{fig:chatgpt_prompts3}
\end{figure*}


==> figs/prompts4.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figs/prompts4_fig.pdf}
    \caption{ChatGPT prompt ensemble 4}
    \label{fig:chatgpt_prompts4}
\end{figure*}


==> figs/prompts5.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figs/prompts5_fig.pdf}
    \caption{ChatGPT prompt ensemble 5}
    \label{fig:chatgpt_prompts5}
\end{figure*}


==> figs/qualitative_ablation_part1.tex <==
% Use figure* for multi-column figure
\begin{figure}[h]
\centering
\begin{minipage}{0.592\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/mvtec_scale_0shot.pdf}
\captionsetup{labelformat=empty,font=small,skip=1pt}
\caption*{(a) 0-shot.}\label{fig:qual_scale_0shot}
\end{minipage}
\hspace{0.000001\linewidth}
\begin{minipage}{0.394\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/mvtec_scale_1shot.pdf}
\captionsetup{labelformat=empty,font=small,skip=1pt}
\caption*{(b) 1-shot.}\label{fig:qual_scale_1shot}
\end{minipage}

\caption{Qualitative AS results for the image scale ablation study on MVTec-AD.}
\label{fig:qualitative_ablation_part1}
\end{figure}

==> figs/qualitative_ablation_part2.tex <==
\begin{figure}[h]
\centering
\begin{minipage}{0.4553\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/mvtec_models_0shot.pdf}
\captionsetup{labelformat=empty,font=small,skip=1pt}
\caption*{(a) MVTec-AD}\label{fig:qual_mvtec_models}
\end{minipage}
\hspace{0.000001\linewidth}
\begin{minipage}{0.5317\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/visa_models_0shot.pdf}
\captionsetup{labelformat=empty,font=small,skip=1pt}
\caption*{(b) VisA}\label{fig:qual_visa_models}
\end{minipage}

\caption{Qualitative results for language- vs vision-guided zero-shot AS.}
\label{fig:qualitative_ablation_part2}
\end{figure}

==> figs/qualitative_additional_main_mvtec.tex <==
\begin{figure}[t]
\centering
\begin{minipage}{0.481\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/mvtec_clip_vs_gem.pdf}
\caption{Qualitative results for impact of CLIP vs GEM patch embeddings on language-guided zero-shot AS on MVTec-AD.}\label{fig:qual_mvtec_clip_vs_gem}
\vspace{2.9em}
\includegraphics[width=\textwidth]{figs/mvtec_shots_study_1.pdf}
\captionsetup{labelformat=empty,font=small,skip=1pt}
\caption*{}\label{fig:qual_mvtec_shots_study_1}
\end{minipage}
\hspace{0.000001\linewidth}
\begin{minipage}{0.48\linewidth}
\includegraphics[width=\textwidth]{figs/mvtec_shots_study_2.pdf}
\captionsetup{labelformat=empty,font=small,skip=1pt}
\caption*{}\label{fig:qual_mvtec_shots_study_2}
\end{minipage}

\caption{Additional qualitative results for zero-shot and one-shot AS on MVTec-AD.}
\label{fig:qualitative_additional_main_mvtec}
\end{figure}

==> figs/qualitative_additional_main_visa.tex <==
\begin{figure}[h]
\centering
\begin{minipage}{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/visa_shots_study_1.pdf}
\captionsetup{labelformat=empty,font=small,skip=1pt}
\caption*{}\label{fig:qual_visa_shots_study_1}
\end{minipage}
\hspace{0.000001\linewidth}
\begin{minipage}{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{figs/visa_shots_study_2.pdf}
\captionsetup{labelformat=empty,font=small,skip=1pt}
\caption*{}\label{fig:qual_visa_shots_study_2}
\end{minipage}

\caption{Additional qualitative results for zero-shot and one-shot AS on VisA.}
\label{fig:qualitative_additional_main_visa}
\end{figure}

==> tables/ablation_clip_vs_gem_as.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{l|cc}
\toprule
Patch embeddings & MVTec-AD & VisA \\
\midrule
CLIP & 18.0 & 13.9  \\
GEM & \textbf{86.5}  & \textbf{87.0} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
CLIP vs GEM patch embeddings for zero-shot AS (pAUROC) on MVTec-AD.
}
\label{tab:ablation_clip_vs_gem_as}
\end{table}

==> tables/ablation_lang_vs_vis_mvtec_ac.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{cccc}
\toprule
\multicolumn{2}{c}{AC (AUROC)} & \multicolumn{2}{c}{\# shots} \\
\cmidrule(r){1-2} \cmidrule(l){3-4}
$s_{lang}$ & $s_{vis}$ & 1     & 4 \\
\cmidrule(r){1-2} \cmidrule(l){3-4}
\ding{51} & \ding{55} & 90.0  & 90.0 \\
\ding{55} & \ding{51} & 90.7  & 94.5 \\
\cmidrule(r){1-2} \cmidrule(l){3-4}
\ding{51} & \ding{51} & \textbf{93.9}  & \textbf{96.3} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Ablations on language- vs vision-guided AC on MVTec-AD.
}
\label{tab:ablation_lang_vs_vis_mvtec_ac}
\end{table}

==> tables/ablation_lang_vs_vis_mvtec_as.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{ccccc}
\toprule
\multicolumn{2}{c}{AS (pAUROC)} & \multicolumn{3}{c}{\# shots} \\
\cmidrule(r){1-2} \cmidrule(l){3-5}
$\boldsymbol{M}^{lang}$ & $\boldsymbol{M}^{vis}$ & 0 & 1     & 4 \\
\cmidrule(r){1-2} \cmidrule(l){3-5}
\ding{51} & \ding{55} & 86.5 & 86.5  & 86.5 \\
\ding{55} & \ding{51} & 86.6 & 95.1  & 96.1 \\
\cmidrule(r){1-2} \cmidrule(l){3-5}
\ding{51} & \ding{51} & \textbf{89.6} & \textbf{95.4}  & \textbf{96.2} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Ablations on language- vs vision-guided AS on MVTec-AD.
}
\label{tab:ablation_lang_vs_vis_mvtec_as}
\end{table}

==> tables/ablation_multiscale_mvtec_ac.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{cccc}
\toprule
AC (AUROC) & \multicolumn{3}{c}{\# shots} \\
\cmidrule(l){2-4}
Image scale & 1     & 2     & 4 \\
\cmidrule(r){1-1} \cmidrule(l){2-4}
240 & 92.6  & 94.4  & 95.3 \\
448 & 92.3  & 93.7  & 94.6 \\
896 & 90.5  & 91.5  & 92.7 \\
\cmidrule(r){1-1} \cmidrule(l){2-4}
Multi-scale & \textbf{93.9}  & \textbf{95.2}  & \textbf{96.3} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Image scale ablations for AC on MVTec-AD.
}
\label{tab:ablation_img_scale_mvtec_ac}
\end{table}

==> tables/ablation_multiscale_mvtec_as.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{ccccc}
\toprule
AS (pAUROC) & \multicolumn{4}{c}{\# shots} \\
\cmidrule(l){2-5}
Image scale & 0     & 1     & 2     & 4 \\
\cmidrule(r){1-1} \cmidrule(l){2-5}
240 & 87.6  & 93.4  & 94.0  & 94.5 \\
448 & 87.4  & 93.5  & 94.0  & 94.5 \\
896 & 84.7  & 91.3  & 91.7  & 92.1 \\
\cmidrule(r){1-1} \cmidrule(l){2-5}
Multi-scale & \textbf{89.6}  & \textbf{95.4}  & \textbf{95.8}  & \textbf{96.2} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Image scale ablations for AS on MVTec-AD.
}
\label{tab:ablation_img_scale_mvtec_as}
\end{table}

==> tables/ablation_prompts.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{l|cc}
\toprule
Prompt ensemble & MVTec-AD & VisA \\
\midrule
WinCLIP prompts & 83.7 & 74.0  \\
WinCLIP + ChatGPT prompts & \textbf{86.5}  & \textbf{87.0} \\
\bottomrule
\end{tabular}
\end{center}
\caption{
Prompt ensemble ablations on zero-shot AS (pAUROC).
}
%\vspace{-0.05in}
\label{tab:ablation_prompts}
\end{table}

==> tables/ac_more_methods.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%

\begin{tabular}{clcccccc}
\toprule
\multicolumn{2}{l}{Anomaly Classification} & \multicolumn{3}{c}{MVTec-AD} & \multicolumn{3}{c}{VisA} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
Setup & Method & AUROC & AUPR & $F1$-max & AUROC & AUPR & $F1$-max\\
\midrule
0-shot & WinCLIP & \red{91.8$\pm$\small{0.0}} & \red{96.5$\pm$\small{0.0}} & \red{92.9$\pm$\small{0.0}} & \blue{78.1$\pm$\small{0.0}} & 81.2$\pm$\small{0.0} & \red{79.0$\pm$\small{0.0}} \\
& AnomalyClip & \blue{91.5$\pm$\small{0.0}} & \blue{96.2$\pm$\small{0.0}} & -- & \red{82.1$\pm$\small{0.0}} & \red{85.4$\pm$\small{0.0}} & -- \\
& APRIL-GAN & 86.1$\pm$\small{0.0} & 93.5$\pm$\small{0.0} & 90.4$\pm$\small{0.0} & 78.0$\pm$\small{0.0} & \blue{81.4$\pm$\small{0.0}} & \blue{78.7$\pm$\small{0.0}} \\
\cmidrule(lr){2-8}
& FADE (ours) & 90.0$\pm$\small{0.0} & 95.6$\pm$\small{0.0} & \blue{92.4$\pm$\small{0.0}} & 75.6$\pm$\small{0.0} & 78.5$\pm$\small{0.0} & 78.6$\pm$\small{0.0} \\
\midrule
1-shot & PatchCore & 83.4$\pm$\small{3.0} & 92.2$\pm$\small{1.5} & 90.5$\pm$\small{1.5} & 79.9$\pm$\small{2.9} & 82.8$\pm$\small{2.3} & 81.7$\pm$\small{1.6} \\
& WinCLIP+ & 93.1$\pm$\small{2.0} & \blue{96.5$\pm$\small{0.9}} & \blue{93.7$\pm$\small{1.1}} & 83.8$\pm$\small{4.0} & 85.1$\pm$\small{4.0} & 83.1$\pm$\small{1.7} \\
& AnomalyGPT & \red{94.1$\pm$\small{1.1}} & -- & -- & \blue{87.4$\pm$\small{0.8}} & -- & -- \\
& APRIL-GAN & 92.0$\pm$\small{0.3} & 95.8$\pm$\small{0.2} & 92.4$\pm$\small{0.2} & \red{91.2$\pm$\small{0.8}} & \red{93.3$\pm$\small{0.8}} & \red{86.9$\pm$\small{0.6}} \\
\cmidrule(lr){2-8}
& FADE (ours) & \blue{93.9$\pm$\small{0.7}} & \red{96.8$\pm$\small{0.3}} & \red{94.8$\pm$\small{0.2}} & 86.7$\pm$\small{2.0} & \blue{87.9$\pm$\small{1.5}} & \blue{84.7$\pm$\small{0.8}} \\
\midrule
2-shot & PatchCore & 86.3$\pm$\small{3.3} & 93.8$\pm$\small{1.7} & 92.0$\pm$\small{1.5} & 81.6$\pm$\small{4.0} & 84.8$\pm$\small{3.2} & 82.5$\pm$\small{1.8} \\
& WinCLIP+ & 94.4$\pm$\small{1.3} & \blue{97.0$\pm$\small{0.7}} & \blue{94.4$\pm$\small{0.8}} & 84.6$\pm$\small{2.4} & 85.8$\pm$\small{2.7} & 83.0$\pm$\small{1.4} \\
& AnomalyGPT & \red{95.5$\pm$\small{0.8}} & -- & -- & 88.6$\pm$\small{0.7} & -- & -- \\
& APRIL-GAN & 92.4$\pm$\small{0.3} & 96.0$\pm$\small{0.2} & 92.6$\pm$\small{0.1} & \red{92.2$\pm$\small{0.3}} & \red{94.2$\pm$\small{0.3}} & \red{87.7$\pm$\small{0.3}} \\
\cmidrule(lr){2-8}
& FADE (ours) & \blue{95.2$\pm$\small{1.0}} & \red{97.6$\pm$\small{0.5}} & \red{95.0$\pm$\small{0.4}} & \blue{89.2$\pm$\small{0.4}} & \blue{90.2$\pm$\small{0.2}} & \blue{85.9$\pm$\small{0.6}} \\
\midrule
4-shot & PatchCore & 88.8$\pm$\small{2.6} & 94.5$\pm$\small{1.5} & 92.6$\pm$\small{1.6} & 85.3$\pm$\small{2.1} & 87.5$\pm$\small{2.1} & 84.3$\pm$\small{1.3} \\
& WinCLIP+ & \blue{95.2$\pm$\small{1.3}} & \blue{97.3$\pm$\small{0.6}} & \blue{94.7$\pm$\small{0.8}} & 87.3$\pm$\small{1.8} & 88.8$\pm$\small{1.8} & 84.2$\pm$\small{1.6} \\
& AnomalyGPT & \red{96.3$\pm$\small{0.3}} & -- & -- & 90.6$\pm$\small{0.7} & -- & -- \\
& APRIL-GAN & 92.8$\pm$\small{0.2} & 96.3$\pm$\small{0.1} & 92.8$\pm$\small{0.1} & \red{92.6$\pm$\small{0.4}} & \red{94.5$\pm$\small{0.3}} & \red{88.4$\pm$\small{0.5}} \\
\cmidrule(lr){2-8}
& FADE (ours) & \red{96.3$\pm$\small{0.4}} & \red{98.1$\pm$\small{0.2}} & \red{95.5$\pm$\small{0.4}} & \blue{90.7$\pm$\small{0.3}} & \blue{91.9$\pm$\small{0.4}} & \blue{87.0$\pm$\small{0.2}} \\
\bottomrule
\end{tabular}

}
\caption{
Additional comparison of AC performance on MVTec-AD and VisA. We report the mean and standard deviation over 5 random seeds. Bold and underline denote the best and second best results respectively. AnomalyCLIP~\cite{zhou2024anomalyclip}, AnomalyGPT~\cite{gu2024anomalygpt} and APRIL-GAN~\cite{chen2023aprilgan} use additional datasets for training. WinCLIP~\cite{jeong2023winclip} and FADE require no training.
}
\label{tab:appendix_ac}
\end{table}

==> tables/as_more_methods.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%

\begin{tabular}{clcccccc}
\toprule
\multicolumn{2}{l}{Anomaly Segmentation} & \multicolumn{3}{c}{MVTec-AD} & \multicolumn{3}{c}{VisA} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
Setup & Method & pAUROC & PRO & $F1$-max & pAUROC & PRO & $F1$-max\\
\midrule
0-shot & WinCLIP & 85.1$\pm$\small{0.0} & 64.6$\pm$\small{0.0} & 31.7$\pm$\small{0.0} & 79.6$\pm$\small{0.0} & 56.8$\pm$\small{0.0} & 14.8$\pm$\small{0.0} \\
& AnomalyCLIP & \red{91.1$\pm$\small{0.0}} & \blue{81.4$\pm$\small{0.0}} & -- & \red{95.5$\pm$\small{0.0}} & \red{87.0$\pm$\small{0.0}} & -- \\
& APRIL-GAN & 87.6$\pm$\small{0.0} & 44.0$\pm$\small{0.0} & \red{43.3$\pm$\small{0.0}} & \blue{94.2$\pm$\small{0.0}} & \blue{86.8$\pm$\small{0.0}} &  \red{32.3$\pm$\small{0.0}} \\
\cmidrule(lr){2-8}
& FADE (ours) & \blue{89.6$\pm$\small{0.0}} & \red{84.5$\pm$\small{0.0}} & \blue{39.8$\pm$\small{0.0}} & 91.5$\pm$\small{0.0} & 79.3$\pm$\small{0.0} & \blue{16.7$\pm$\small{0.0}} \\
\midrule
1-shot & PatchCore & 92.0$\pm$\small{1.0} & 79.7$\pm$\small{2.0} & 50.4$\pm$\small{2.1} & 95.4$\pm$\small{0.6} & 80.5$\pm$\small{2.5} & 38.0$\pm$\small{1.9} \\
& WinCLIP+ & 95.2$\pm$\small{0.5} & 87.1$\pm$\small{1.2} & \red{55.9$\pm$\small{2.7}} & \blue{96.4$\pm$\small{0.4}} & 85.1$\pm$\small{2.1} & \blue{41.3$\pm$\small{2.3}} \\
& AnomalyGPT & \blue{95.3$\pm$\small{0.1}} & -- & -- & 96.2$\pm$\small{0.1} & -- & -- \\
& APRIL-GAN & 95.1$\pm$\small{0.1} & \red{90.6$\pm$\small{0.2}} & 54.2$\pm$\small{0.0} & 96.0$\pm$\small{0.0} & \red{90.0$\pm$\small{0.1}} & 38.5$\pm$\small{0.3} \\
\cmidrule(lr){2-8}
& FADE (ours) & \red{95.4$\pm$\small{0.3}} & \blue{88.3$\pm$\small{0.3}} & \blue{54.6$\pm$\small{1.1}} & \red{97.5$\pm$\small{0.1}} & \blue{88.9$\pm$\small{0.7}} & \red{42.3$\pm$\small{0.5}} \\
\midrule
2-shot & PatchCore & 93.3$\pm$\small{0.6} & 82.3$\pm$\small{1.3} & 53.0$\pm$\small{1.7} & 96.1$\pm$\small{0.5} & 82.6$\pm$\small{2.3} & 41.0$\pm$\small{3.9} \\
& WinCLIP+ & \red{96.0$\pm$\small{0.3}} & 88.4$\pm$\small{0.9} & \red{58.4$\pm$\small{1.7}} & \blue{96.8$\pm$\small{0.3}} & 86.2$\pm$\small{1.4} & \blue{43.5$\pm$\small{3.3}} \\
& AnomalyGPT & 95.6$\pm$\small{0.2} & -- & -- & 96.4$\pm$\small{0.1} & -- & -- \\
& APRIL-GAN & 95.5$\pm$\small{0.0} & \red{91.3$\pm$\small{0.1}} & \blue{55.9$\pm$\small{0.5}} & 96.2$\pm$\small{0.0} & \red{90.1$\pm$\small{0.1}} & 39.3$\pm$\small{0.2} \\
\cmidrule(lr){2-8}
& FADE (ours) & \blue{95.8$\pm$\small{0.2}} & \blue{88.9$\pm$\small{0.2}} & 55.8$\pm$\small{1.0} & \red{97.8$\pm$\small{0.1}} & \blue{89.8$\pm$\small{0.4}} & \red{44.4$\pm$\small{0.9}} \\
\midrule
4-shot & PatchCore & 94.3$\pm$\small{0.5} & 84.3$\pm$\small{1.6} & 55.0$\pm$\small{1.9} & 96.8$\pm$\small{0.3} & 84.9$\pm$\small{1.4} & 43.9$\pm$\small{3.1} \\
& WinCLIP+ & \red{96.2$\pm$\small{0.3}} & 89.0$\pm$\small{0.8} & \red{59.5$\pm$\small{1.8}} & \blue{97.2$\pm$\small{0.2}} & 87.6$\pm$\small{0.9} & \red{47.0$\pm$\small{3.0}} \\
& AnomalyGPT & \red{96.2$\pm$\small{0.1}} & -- & -- & 96.7$\pm$\small{0.1} & -- & -- \\
& APRIL-GAN & \blue{95.9$\pm$\small{0.0}} & \red{91.8$\pm$\small{0.1}} & 56.9$\pm$\small{0.1} & 96.2$\pm$\small{0.0} & \red{90.2$\pm$\small{0.1}} & 40.0$\pm$\small{0.1} \\
\cmidrule(lr){2-8}
& FADE (ours) & \red{96.2$\pm$\small{0.1}} & \blue{89.5$\pm$\small{0.2}} & \blue{57.0$\pm$\small{0.8}} & \red{98.0$\pm$\small{0.0}} & \blue{90.0$\pm$\small{0.4}} & \blue{46.4$\pm$\small{0.7}} \\
\bottomrule
\end{tabular}

}
\caption{
Additional comparison of AS performance on MVTec-AD and VisA. We report the mean and standard deviation over 5 random seeds. Bold and underline denote the best and second best results respectively. AnomalyCLIP~\cite{zhou2024anomalyclip}, AnomalyGPT~\cite{gu2024anomalygpt} and APRIL-GAN~\cite{chen2023aprilgan} use additional datasets for training. WinCLIP~\cite{jeong2023winclip} and FADE require no training.
}
\label{tab:appendix_as}
\end{table}


==> tables/classlevel/ac_mvtec_aupr.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.73\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
MVTec-AD (AC) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    AUPR &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Bottle &  99.8$\pm$\small{0.0} &  99.3$\pm$\small{0.0} &  99.4$\pm$\small{0.3} &  99.8$\pm$\small{0.0} &  99.8$\pm$\small{0.1} &  99.8$\pm$\small{0.1} &  99.8$\pm$\small{0.1} &  99.9$\pm$\small{0.1} \\
     Cable &  91.2$\pm$\small{0.0} &  90.4$\pm$\small{0.0} &  93.2$\pm$\small{1.1} &  95.6$\pm$\small{1.6} &  92.9$\pm$\small{0.6} &  97.2$\pm$\small{1.1} &  94.4$\pm$\small{0.3} &  97.8$\pm$\small{0.1} \\
   Capsule &  91.5$\pm$\small{0.0} &  90.0$\pm$\small{0.0} &  91.6$\pm$\small{2.7} &  89.7$\pm$\small{4.8} &  93.3$\pm$\small{3.6} &  93.7$\pm$\small{5.6} &  95.1$\pm$\small{3.3} &  97.9$\pm$\small{0.4} \\
    Carpet & 100.0$\pm$\small{0.0} &  99.8$\pm$\small{0.0} &  99.9$\pm$\small{0.1} & 100.0$\pm$\small{0.0} &  99.9$\pm$\small{0.1} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} \\
      Grid &  99.6$\pm$\small{0.0} &  99.8$\pm$\small{0.0} &  99.9$\pm$\small{0.1} &  99.6$\pm$\small{0.4} &  99.8$\pm$\small{0.1} &  99.6$\pm$\small{0.3} &  99.9$\pm$\small{0.0} &  99.5$\pm$\small{0.2} \\
  Hazelnut &  96.9$\pm$\small{0.0} &  96.2$\pm$\small{0.0} &  98.6$\pm$\small{0.7} &  98.6$\pm$\small{0.6} &  99.1$\pm$\small{0.4} &  98.8$\pm$\small{0.3} &  99.1$\pm$\small{0.2} &  98.9$\pm$\small{0.4} \\
   Leather & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} \\
 Metal nut &  99.3$\pm$\small{0.0} &  98.9$\pm$\small{0.0} &  99.7$\pm$\small{0.2} &  99.8$\pm$\small{0.0} &  99.9$\pm$\small{0.0} &  99.8$\pm$\small{0.0} &  99.9$\pm$\small{0.1} &  99.9$\pm$\small{0.0} \\
      Pill &  95.7$\pm$\small{0.0} &  96.4$\pm$\small{0.0} &  98.3$\pm$\small{0.5} &  99.1$\pm$\small{0.1} &  98.6$\pm$\small{0.1} &  99.3$\pm$\small{0.1} &  98.6$\pm$\small{0.2} &  99.2$\pm$\small{0.1} \\
     Screw &  93.1$\pm$\small{0.0} &  89.8$\pm$\small{0.0} &  94.2$\pm$\small{0.6} &  88.1$\pm$\small{3.5} &  94.1$\pm$\small{1.5} &  92.1$\pm$\small{2.2} &  94.9$\pm$\small{0.8} &  91.9$\pm$\small{2.9} \\
      Tile & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.1} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} \\
Toothbrush &  95.6$\pm$\small{0.0} &  93.3$\pm$\small{0.0} &  96.7$\pm$\small{2.0} &  97.3$\pm$\small{1.2} &  99.0$\pm$\small{0.6} &  97.4$\pm$\small{0.9} &  98.7$\pm$\small{1.1} &  98.0$\pm$\small{0.8} \\
Transistor &  87.1$\pm$\small{0.0} &  83.6$\pm$\small{0.0} &  79.0$\pm$\small{4.0} &  85.9$\pm$\small{0.4} &  80.7$\pm$\small{2.3} &  87.7$\pm$\small{1.9} &  80.7$\pm$\small{3.2} &  88.9$\pm$\small{1.9} \\
      Wood &  99.8$\pm$\small{0.0} &  99.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} &  99.7$\pm$\small{0.1} & 100.0$\pm$\small{0.0} &  99.8$\pm$\small{0.1} &  99.9$\pm$\small{0.1} &  99.8$\pm$\small{0.1} \\
    Zipper &  97.5$\pm$\small{0.0} &  97.2$\pm$\small{0.0} &  96.8$\pm$\small{1.8} &  99.3$\pm$\small{0.4} &  98.3$\pm$\small{0.4} &  99.3$\pm$\small{0.3} &  98.5$\pm$\small{0.2} &  99.4$\pm$\small{0.5} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean &  \textbf{96.5$\pm$\small{0.0}} &  95.6$\pm$\small{0.0} &  96.5$\pm$\small{0.9} &  \textbf{96.8$\pm$\small{0.3}} &  97.0$\pm$\small{0.7} &  \textbf{97.6$\pm$\small{0.5}} &  97.3$\pm$\small{0.6} &  \textbf{98.1$\pm$\small{0.2}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly classification (AC) performance in terms of class-wise AUPR on MVTec-AD. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_ac_mvtec_aupr}
\end{table*}


==> tables/classlevel/ac_mvtec_auroc.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.73\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
MVTec-AD (AC) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    AUROC &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Bottle &  99.2$\pm$\small{0.0} &  97.7$\pm$\small{0.0} & 98.2$\pm$\small{0.9} &  99.3$\pm$\small{0.1} & 99.3$\pm$\small{0.3} &  99.4$\pm$\small{0.3} &  99.3$\pm$\small{0.4} &  99.8$\pm$\small{0.4} \\
     Cable &  86.5$\pm$\small{0.0} &  85.5$\pm$\small{0.0} & 88.9$\pm$\small{1.9} &  93.1$\pm$\small{2.0} & 88.4$\pm$\small{0.7} &  95.1$\pm$\small{1.4} &  90.9$\pm$\small{0.9} &  96.1$\pm$\small{0.3} \\
   Capsule &  72.9$\pm$\small{0.0} &  67.8$\pm$\small{0.0} & 72.3$\pm$\small{6.8} & 71.5$\pm$\small{11.3} & 77.3$\pm$\small{8.8} & 80.3$\pm$\small{13.2} &  82.3$\pm$\small{8.9} &  91.0$\pm$\small{1.9} \\
    Carpet & 100.0$\pm$\small{0.0} &  99.3$\pm$\small{0.0} & 99.8$\pm$\small{0.3} &  99.9$\pm$\small{0.1} & 99.8$\pm$\small{0.3} & 100.0$\pm$\small{0.1} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} \\
      Grid &  98.8$\pm$\small{0.0} &  99.4$\pm$\small{0.0} & 99.5$\pm$\small{0.3} &  98.8$\pm$\small{1.4} & 99.4$\pm$\small{0.2} &  99.0$\pm$\small{0.8} &  99.6$\pm$\small{0.1} &  98.6$\pm$\small{0.7} \\
  Hazelnut &  93.9$\pm$\small{0.0} &  92.6$\pm$\small{0.0} & 97.5$\pm$\small{1.4} &  97.3$\pm$\small{1.2} & 98.3$\pm$\small{0.7} &  97.6$\pm$\small{0.6} &  98.4$\pm$\small{0.4} &  97.8$\pm$\small{0.7} \\
   Leather & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 99.9$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 99.9$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} \\
 Metal nut &  97.1$\pm$\small{0.0} &  95.5$\pm$\small{0.0} & 98.7$\pm$\small{0.8} &  99.0$\pm$\small{0.2} & 99.4$\pm$\small{0.2} &  99.2$\pm$\small{0.2} &  99.5$\pm$\small{0.2} &  99.3$\pm$\small{0.2} \\
      Pill &  79.1$\pm$\small{0.0} &  81.6$\pm$\small{0.0} & 91.2$\pm$\small{2.1} &  95.3$\pm$\small{0.6} & 92.3$\pm$\small{0.7} &  95.9$\pm$\small{0.7} &  92.8$\pm$\small{1.0} &  95.8$\pm$\small{0.4} \\
     Screw &  83.3$\pm$\small{0.0} &  74.9$\pm$\small{0.0} & 86.4$\pm$\small{0.9} &  75.9$\pm$\small{5.1} & 86.0$\pm$\small{2.1} &  82.0$\pm$\small{3.2} &  87.9$\pm$\small{1.2} &  82.3$\pm$\small{3.9} \\
      Tile & 100.0$\pm$\small{0.0} &  99.9$\pm$\small{0.0} & 99.9$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 99.9$\pm$\small{0.2} & 100.0$\pm$\small{0.0} &  99.9$\pm$\small{0.1} & 100.0$\pm$\small{0.0} \\
Toothbrush &  87.5$\pm$\small{0.0} &  82.5$\pm$\small{0.0} & 92.2$\pm$\small{4.9} &  92.8$\pm$\small{3.2} & 97.5$\pm$\small{1.6} &  93.1$\pm$\small{2.2} &  96.7$\pm$\small{2.6} &  94.7$\pm$\small{2.1} \\
Transistor &  88.0$\pm$\small{0.0} &  86.4$\pm$\small{0.0} & 83.4$\pm$\small{3.8} &  88.9$\pm$\small{0.5} & 85.3$\pm$\small{1.7} &  90.2$\pm$\small{2.0} &  85.7$\pm$\small{2.5} &  91.3$\pm$\small{1.5} \\
      Wood &  99.4$\pm$\small{0.0} &  96.7$\pm$\small{0.0} & 99.9$\pm$\small{0.1} &  99.1$\pm$\small{0.3} & 99.9$\pm$\small{0.1} &  99.3$\pm$\small{0.4} &  99.8$\pm$\small{0.3} &  99.4$\pm$\small{0.2} \\
    Zipper &  91.5$\pm$\small{0.0} &  90.5$\pm$\small{0.0} & 88.8$\pm$\small{5.9} &  97.7$\pm$\small{1.2} & 94.0$\pm$\small{1.4} &  97.5$\pm$\small{1.0} &  94.5$\pm$\small{0.5} &  97.9$\pm$\small{1.7} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean &  \textbf{91.8$\pm$\small{0.0}} &  90.0$\pm$\small{0.0} & 93.1$\pm$\small{2.0} &  \textbf{93.9$\pm$\small{0.7}} & 94.4$\pm$\small{1.3} &  \textbf{95.2$\pm$\small{1.0}} &  95.2$\pm$\small{1.3} &  \textbf{96.3$\pm$\small{0.4}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly classification (AC) performance in terms of class-wise AUROC on MVTec-AD. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_ac_mvtec_auroc}
\end{table*}


==> tables/classlevel/ac_mvtec_f1_max.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.73\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
MVTec-AD (AC) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    $F_1$-max &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
        Bottle &  97.6$\pm$\small{0.0} &  96.1$\pm$\small{0.0} & 96.5$\pm$\small{1.3} &  98.4$\pm$\small{0.0} & 97.7$\pm$\small{0.7} &  98.3$\pm$\small{0.7} & 97.8$\pm$\small{0.6} &  98.9$\pm$\small{1.2} \\
     Cable &  84.5$\pm$\small{0.0} &  86.2$\pm$\small{0.0} & 86.1$\pm$\small{1.3} &  90.2$\pm$\small{1.6} & 85.2$\pm$\small{0.7} &  91.4$\pm$\small{1.7} & 87.2$\pm$\small{0.6} &  92.6$\pm$\small{0.8} \\
   Capsule &  91.4$\pm$\small{0.0} &  93.0$\pm$\small{0.0} & 91.6$\pm$\small{0.7} &  93.2$\pm$\small{0.8} & 92.1$\pm$\small{0.7} &  93.5$\pm$\small{1.3} & 92.5$\pm$\small{0.5} &  94.5$\pm$\small{1.0} \\
    Carpet &  99.4$\pm$\small{0.0} &  97.8$\pm$\small{0.0} & 99.2$\pm$\small{0.8} &  99.7$\pm$\small{0.3} & 99.3$\pm$\small{0.7} &  99.8$\pm$\small{0.3} & 99.9$\pm$\small{0.2} &  99.7$\pm$\small{0.3} \\
      Grid &  98.2$\pm$\small{0.0} &  98.2$\pm$\small{0.0} & 98.9$\pm$\small{0.4} &  98.4$\pm$\small{1.2} & 99.1$\pm$\small{0.0} &  97.7$\pm$\small{1.6} & 99.1$\pm$\small{0.0} &  97.3$\pm$\small{1.1} \\
  Hazelnut &  89.7$\pm$\small{0.0} &  88.6$\pm$\small{0.0} & 94.7$\pm$\small{2.3} &  94.4$\pm$\small{1.8} & 95.6$\pm$\small{1.6} &  94.3$\pm$\small{1.3} & 96.2$\pm$\small{1.0} &  95.0$\pm$\small{0.9} \\
   Leather & 100.0$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 99.5$\pm$\small{0.0} & 100.0$\pm$\small{0.0} & 99.7$\pm$\small{0.2} & 100.0$\pm$\small{0.0} & 99.8$\pm$\small{0.2} & 100.0$\pm$\small{0.0} \\
 Metal nut &  96.3$\pm$\small{0.0} &  95.1$\pm$\small{0.0} & 97.7$\pm$\small{1.0} &  98.5$\pm$\small{0.6} & 98.4$\pm$\small{0.5} &  98.7$\pm$\small{0.3} & 98.5$\pm$\small{0.6} &  99.2$\pm$\small{0.3} \\
      Pill &  91.6$\pm$\small{0.0} &  91.6$\pm$\small{0.0} & 93.8$\pm$\small{0.7} &  95.3$\pm$\small{0.5} & 94.3$\pm$\small{0.4} &  95.4$\pm$\small{0.5} & 94.1$\pm$\small{0.4} &  95.3$\pm$\small{0.4} \\
     Screw &  87.4$\pm$\small{0.0} &  86.1$\pm$\small{0.0} & 88.5$\pm$\small{0.3} &  87.4$\pm$\small{0.9} & 89.0$\pm$\small{0.6} &  87.9$\pm$\small{1.0} & 89.6$\pm$\small{0.7} &  88.4$\pm$\small{1.2} \\
      Tile &  99.4$\pm$\small{0.0} &  99.4$\pm$\small{0.0} & 98.9$\pm$\small{0.2} &  99.9$\pm$\small{0.3} & 99.2$\pm$\small{0.3} & 100.0$\pm$\small{0.0} & 99.2$\pm$\small{0.3} & 100.0$\pm$\small{0.0} \\
Toothbrush &  87.9$\pm$\small{0.0} &  87.5$\pm$\small{0.0} & 94.1$\pm$\small{1.9} &  92.1$\pm$\small{2.6} & 96.7$\pm$\small{1.8} &  91.7$\pm$\small{2.7} & 96.8$\pm$\small{2.3} &  93.0$\pm$\small{2.6} \\
Transistor &  79.5$\pm$\small{0.0} &  78.3$\pm$\small{0.0} & 75.1$\pm$\small{3.1} &  78.6$\pm$\small{0.8} & 75.9$\pm$\small{2.4} &  81.2$\pm$\small{3.0} & 76.6$\pm$\small{2.8} &  82.8$\pm$\small{2.9} \\
      Wood &  98.3$\pm$\small{0.0} &  95.2$\pm$\small{0.0} & 99.4$\pm$\small{0.3} &  97.7$\pm$\small{0.7} & 99.5$\pm$\small{0.4} &  98.3$\pm$\small{0.6} & 99.2$\pm$\small{0.9} &  98.2$\pm$\small{0.4} \\
    Zipper &  92.9$\pm$\small{0.0} &  92.7$\pm$\small{0.0} & 92.1$\pm$\small{2.5} &  97.6$\pm$\small{1.1} & 94.4$\pm$\small{0.3} &  96.9$\pm$\small{0.7} & 94.7$\pm$\small{0.4} &  97.6$\pm$\small{1.1} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean &  \textbf{92.9$\pm$\small{0.0}} &  92.4$\pm$\small{0.0} & 93.7$\pm$\small{1.1} &  \textbf{94.8$\pm$\small{0.2}} & 94.4$\pm$\small{0.8} &  \textbf{95.0$\pm$\small{0.4}} & 94.7$\pm$\small{0.8} &  \textbf{95.5$\pm$\small{0.4}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly classification (AC) performance in terms of class-wise $F_1$-max on MVTec-AD. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_ac_mvtec_f1_max}
\end{table*}


==> tables/classlevel/ac_visa_aupr.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
VisA (AC) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    AUPR &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Candle & 95.8$\pm$\small{0.0} & 95.4$\pm$\small{0.0} &  93.6$\pm$\small{1.5} &  96.1$\pm$\small{1.3} &  95.1$\pm$\small{1.1} & 96.6$\pm$\small{0.7} & 95.3$\pm$\small{0.4} & 97.0$\pm$\small{0.7} \\
  Capsules & 90.9$\pm$\small{0.0} & 87.9$\pm$\small{0.0} &  89.9$\pm$\small{2.5} &  89.7$\pm$\small{1.1} &  88.9$\pm$\small{0.7} & 90.5$\pm$\small{1.3} & 91.5$\pm$\small{1.4} & 91.2$\pm$\small{1.2} \\
    Cashew & 96.4$\pm$\small{0.0} & 96.1$\pm$\small{0.0} &  97.2$\pm$\small{0.2} &  97.2$\pm$\small{0.6} &  97.3$\pm$\small{0.2} & 97.5$\pm$\small{0.3} & 97.7$\pm$\small{0.4} & 97.8$\pm$\small{0.3} \\
Chewinggum & 98.6$\pm$\small{0.0} & 98.0$\pm$\small{0.0} &  99.0$\pm$\small{0.3} &  99.0$\pm$\small{0.2} &  98.9$\pm$\small{0.3} & 99.2$\pm$\small{0.2} & 99.0$\pm$\small{0.1} & 99.2$\pm$\small{0.2} \\
     Fryum & 90.1$\pm$\small{0.0} & 87.0$\pm$\small{0.0} &  94.7$\pm$\small{1.0} &  97.0$\pm$\small{0.7} &  95.8$\pm$\small{0.2} & 97.3$\pm$\small{0.4} & 96.0$\pm$\small{0.3} & 97.9$\pm$\small{0.1} \\
 Macaroni1 & 75.8$\pm$\small{0.0} & 79.0$\pm$\small{0.0} &  84.9$\pm$\small{1.2} &  92.2$\pm$\small{2.2} &  84.7$\pm$\small{1.5} & 94.2$\pm$\small{1.1} & 86.5$\pm$\small{0.6} & 94.0$\pm$\small{0.4} \\
 Macaroni2 & 60.3$\pm$\small{0.0} & 64.9$\pm$\small{0.0} &  68.4$\pm$\small{1.8} &  69.6$\pm$\small{4.5} &  70.4$\pm$\small{1.8} & 69.8$\pm$\small{3.4} & 69.6$\pm$\small{2.8} & 73.4$\pm$\small{2.5} \\
      PCB1 & 78.4$\pm$\small{0.0} & 73.5$\pm$\small{0.0} & 76.5$\pm$\small{19.0} &  87.4$\pm$\small{3.6} &  78.3$\pm$\small{4.3} & 87.3$\pm$\small{3.2} & 87.7$\pm$\small{1.7} & 90.7$\pm$\small{2.7} \\
      PCB2 & 49.2$\pm$\small{0.0} & 45.3$\pm$\small{0.0} &  64.9$\pm$\small{3.3} &  73.1$\pm$\small{1.7} &  65.8$\pm$\small{4.0} & 76.9$\pm$\small{1.9} & 71.3$\pm$\small{3.4} & 81.3$\pm$\small{0.9} \\
      PCB3 & 76.5$\pm$\small{0.0} & 63.9$\pm$\small{0.0} &  73.5$\pm$\small{1.6} &  79.8$\pm$\small{5.3} &  80.9$\pm$\small{1.6} & 84.2$\pm$\small{2.6} & 84.8$\pm$\small{1.8} & 87.8$\pm$\small{2.8} \\
      PCB4 & 77.7$\pm$\small{0.0} & 69.1$\pm$\small{0.0} & 78.5$\pm$\small{15.5} & 76.1$\pm$\small{21.7} & 72.5$\pm$\small{16.2} & 90.7$\pm$\small{3.4} & 85.6$\pm$\small{8.9} & 93.5$\pm$\small{1.3} \\
Pipe fryum & 82.3$\pm$\small{0.0} & 81.6$\pm$\small{0.0} &  98.6$\pm$\small{0.5} &  97.4$\pm$\small{2.1} &  99.0$\pm$\small{0.3} & 98.0$\pm$\small{1.4} & 99.2$\pm$\small{0.2} & 98.4$\pm$\small{0.5} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & \textbf{81.2$\pm$\small{0.0}} & 78.5$\pm$\small{0.0} &  85.1$\pm$\small{4.0} &  \textbf{87.9$\pm$\small{1.5}} &  85.8$\pm$\small{2.7} & \textbf{90.2$\pm$\small{0.2}} & 88.8$\pm$\small{1.8} & \textbf{91.9$\pm$\small{0.4}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly classification (AC) performance in terms of class-wise AUPR on VisA. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_ac_visa_aupr}
\end{table*}


==> tables/classlevel/ac_visa_auroc.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
VisA (AC) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    AUROC &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
Candle & 95.4$\pm$\small{0.0} & 94.7$\pm$\small{0.0} &  93.4$\pm$\small{1.4} &  95.7$\pm$\small{1.6} & 94.8$\pm$\small{1.0} & 96.3$\pm$\small{0.8} & 95.1$\pm$\small{0.3} & 96.6$\pm$\small{0.6} \\
  Capsules & 85.0$\pm$\small{0.0} & 79.8$\pm$\small{0.0} &  85.0$\pm$\small{3.1} &  83.8$\pm$\small{1.7} & 84.9$\pm$\small{0.8} & 84.9$\pm$\small{1.8} & 86.8$\pm$\small{1.7} & 85.3$\pm$\small{1.7} \\
    Cashew & 92.1$\pm$\small{0.0} & 91.6$\pm$\small{0.0} &  94.0$\pm$\small{0.4} &  94.1$\pm$\small{1.1} & 94.3$\pm$\small{0.5} & 94.8$\pm$\small{0.6} & 95.2$\pm$\small{0.8} & 95.4$\pm$\small{0.7} \\
Chewinggum & 96.5$\pm$\small{0.0} & 95.4$\pm$\small{0.0} &  97.6$\pm$\small{0.8} &  97.5$\pm$\small{0.6} & 97.3$\pm$\small{0.8} & 98.0$\pm$\small{0.3} & 97.7$\pm$\small{0.3} & 98.2$\pm$\small{0.4} \\
     Fryum & 80.3$\pm$\small{0.0} & 73.8$\pm$\small{0.0} &  88.5$\pm$\small{1.9} &  93.3$\pm$\small{1.4} & 90.5$\pm$\small{0.4} & 94.0$\pm$\small{0.8} & 90.8$\pm$\small{0.5} & 95.1$\pm$\small{0.2} \\
 Macaroni1 & 76.2$\pm$\small{0.0} & 78.4$\pm$\small{0.0} &  82.9$\pm$\small{1.5} &  90.7$\pm$\small{3.4} & 83.3$\pm$\small{1.9} & 93.5$\pm$\small{1.5} & 85.2$\pm$\small{0.9} & 93.2$\pm$\small{0.6} \\
 Macaroni2 & 63.7$\pm$\small{0.0} & 66.9$\pm$\small{0.0} &  70.2$\pm$\small{0.9} &  70.3$\pm$\small{4.8} & 71.8$\pm$\small{2.0} & 71.2$\pm$\small{3.6} & 70.9$\pm$\small{2.2} & 74.7$\pm$\small{2.3} \\
      PCB1 & 73.6$\pm$\small{0.0} & 73.0$\pm$\small{0.0} & 75.6$\pm$\small{23.0} &  88.8$\pm$\small{2.6} & 76.7$\pm$\small{5.2} & 88.4$\pm$\small{2.3} & 88.3$\pm$\small{1.7} & 91.0$\pm$\small{1.9} \\
      PCB2 & 51.2$\pm$\small{0.0} & 46.8$\pm$\small{0.0} &  62.2$\pm$\small{3.9} &  73.6$\pm$\small{2.0} & 62.6$\pm$\small{3.7} & 76.7$\pm$\small{1.5} & 67.5$\pm$\small{2.6} & 80.7$\pm$\small{0.6} \\
      PCB3 & 73.4$\pm$\small{0.0} & 64.6$\pm$\small{0.0} &  74.1$\pm$\small{1.1} &  78.3$\pm$\small{5.8} & 78.8$\pm$\small{1.9} & 82.6$\pm$\small{2.3} & 83.3$\pm$\small{1.7} & 86.3$\pm$\small{2.6} \\
      PCB4 & 79.6$\pm$\small{0.0} & 75.4$\pm$\small{0.0} &  85.2$\pm$\small{8.9} & 79.4$\pm$\small{24.8} & 82.3$\pm$\small{9.9} & 93.5$\pm$\small{3.4} & 87.6$\pm$\small{8.0} & 95.4$\pm$\small{0.5} \\
Pipe fryum & 69.7$\pm$\small{0.0} & 67.2$\pm$\small{0.0} &  97.2$\pm$\small{1.1} &  95.2$\pm$\small{3.7} & 98.0$\pm$\small{0.6} & 96.1$\pm$\small{2.6} & 98.5$\pm$\small{0.4} & 96.8$\pm$\small{1.0} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & \textbf{78.1$\pm$\small{0.0}} & 75.6$\pm$\small{0.0} &  83.8$\pm$\small{4.0} &  \textbf{86.7$\pm$\small{2.0}} & 84.6$\pm$\small{2.4} & \textbf{89.2$\pm$\small{0.4}} & 87.3$\pm$\small{1.8} & \textbf{90.7$\pm$\small{0.3}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly classification (AC) performance in terms of class-wise AUROC on VisA. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_ac_visa_auroc}
\end{table*}


==> tables/classlevel/ac_visa_f1_max.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
VisA (AC) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    $F_1$-max &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Candle & 89.4$\pm$\small{0.0} & 90.5$\pm$\small{0.0} & 87.8$\pm$\small{1.2} &  89.3$\pm$\small{2.3} & 89.1$\pm$\small{1.3} & 90.5$\pm$\small{1.9} & 88.9$\pm$\small{1.0} & 90.3$\pm$\small{1.7} \\
  Capsules & 83.9$\pm$\small{0.0} & 82.0$\pm$\small{0.0} & 84.9$\pm$\small{2.0} &  84.0$\pm$\small{1.4} & 85.4$\pm$\small{0.6} & 84.1$\pm$\small{0.9} & 86.0$\pm$\small{0.9} & 84.2$\pm$\small{1.3} \\
    Cashew & 88.4$\pm$\small{0.0} & 89.8$\pm$\small{0.0} & 90.7$\pm$\small{0.7} &  90.8$\pm$\small{0.9} & 90.9$\pm$\small{0.7} & 91.8$\pm$\small{0.8} & 91.6$\pm$\small{1.3} & 92.2$\pm$\small{1.4} \\
Chewinggum & 94.8$\pm$\small{0.0} & 92.6$\pm$\small{0.0} & 95.6$\pm$\small{0.9} &  95.7$\pm$\small{0.6} & 95.4$\pm$\small{0.6} & 96.0$\pm$\small{0.8} & 95.7$\pm$\small{0.5} & 96.3$\pm$\small{0.6} \\
     Fryum & 82.7$\pm$\small{0.0} & 80.2$\pm$\small{0.0} & 87.2$\pm$\small{1.4} &  91.3$\pm$\small{2.0} & 88.4$\pm$\small{0.6} & 91.4$\pm$\small{1.2} & 88.9$\pm$\small{0.8} & 92.6$\pm$\small{0.3} \\
 Macaroni1 & 74.2$\pm$\small{0.0} & 74.9$\pm$\small{0.0} & 76.2$\pm$\small{1.4} &  83.6$\pm$\small{2.8} & 76.7$\pm$\small{2.0} & 86.2$\pm$\small{2.3} & 78.2$\pm$\small{1.2} & 85.8$\pm$\small{0.9} \\
 Macaroni2 & 69.8$\pm$\small{0.0} & 69.0$\pm$\small{0.0} & 72.3$\pm$\small{1.1} &  71.1$\pm$\small{2.2} & 73.9$\pm$\small{0.9} & 71.5$\pm$\small{2.7} & 73.1$\pm$\small{1.6} & 72.8$\pm$\small{1.6} \\
      PCB1 & 71.0$\pm$\small{0.0} & 72.2$\pm$\small{0.0} & 81.3$\pm$\small{6.6} &  85.1$\pm$\small{0.6} & 73.2$\pm$\small{3.7} & 84.3$\pm$\small{1.7} & 83.1$\pm$\small{2.2} & 86.0$\pm$\small{1.7} \\
      PCB2 & 67.1$\pm$\small{0.0} & 67.4$\pm$\small{0.0} & 67.2$\pm$\small{0.3} &  72.9$\pm$\small{2.0} & 67.3$\pm$\small{0.3} & 73.7$\pm$\small{0.9} & 67.7$\pm$\small{0.6} & 76.1$\pm$\small{1.4} \\
      PCB3 & 71.0$\pm$\small{0.0} & 67.8$\pm$\small{0.0} & 73.5$\pm$\small{1.5} &  74.9$\pm$\small{3.5} & 73.9$\pm$\small{1.3} & 76.6$\pm$\small{2.5} & 77.0$\pm$\small{1.4} & 80.1$\pm$\small{2.3} \\
      PCB4 & 74.9$\pm$\small{0.0} & 76.6$\pm$\small{0.0} & 86.1$\pm$\small{2.1} & 84.6$\pm$\small{10.3} & 86.8$\pm$\small{3.8} & 90.5$\pm$\small{3.7} & 84.6$\pm$\small{7.0} & 93.1$\pm$\small{1.2} \\
Pipe fryum & 80.7$\pm$\small{0.0} & 81.0$\pm$\small{0.0} & 94.4$\pm$\small{0.7} &  93.8$\pm$\small{2.2} & 95.4$\pm$\small{0.8} & 94.5$\pm$\small{2.2} & 95.6$\pm$\small{0.7} & 94.4$\pm$\small{1.6} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & \textbf{79.0$\pm$\small{0.0}} & 78.6$\pm$\small{0.0} & 83.1$\pm$\small{1.7} &  \textbf{84.7$\pm$\small{0.8}} & 83.0$\pm$\small{1.4} & \textbf{85.9$\pm$\small{0.6}} & 84.2$\pm$\small{1.6} & \textbf{87.0$\pm$\small{0.2}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly classification (AC) performance in terms of class-wise $F_1$-max on VisA. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_ac_visa_f1_max}
\end{table*}


==> tables/classlevel/as_mvtec_f1_max.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.73\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
MVTec-AD (AS) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    $F_1$-max &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Bottle & 58.1$\pm$\small{0.0} & 50.8$\pm$\small{0.0} & 72.8$\pm$\small{0.8} & 67.5$\pm$\small{1.2} & 73.2$\pm$\small{0.9} & 68.0$\pm$\small{0.6} & 73.3$\pm$\small{0.6} & 67.9$\pm$\small{0.9} \\
     Cable & 19.7$\pm$\small{0.0} & 20.5$\pm$\small{0.0} & 49.4$\pm$\small{3.3} & 53.5$\pm$\small{1.4} & 51.2$\pm$\small{1.3} & 55.4$\pm$\small{0.7} & 54.7$\pm$\small{1.1} & 56.7$\pm$\small{1.1} \\
   Capsule & 21.7$\pm$\small{0.0} & 21.7$\pm$\small{0.0} & 29.7$\pm$\small{7.8} & 30.0$\pm$\small{6.9} & 43.5$\pm$\small{1.4} & 36.6$\pm$\small{9.3} & 40.7$\pm$\small{4.9} & 43.9$\pm$\small{0.7} \\
    Carpet & 49.7$\pm$\small{0.0} & 72.3$\pm$\small{0.0} & 73.3$\pm$\small{1.5} & 72.1$\pm$\small{0.6} & 72.9$\pm$\small{1.3} & 71.8$\pm$\small{0.8} & 72.0$\pm$\small{0.7} & 71.3$\pm$\small{0.6} \\
      Grid & 18.6$\pm$\small{0.0} & 46.4$\pm$\small{0.0} & 50.7$\pm$\small{4.5} & 42.1$\pm$\small{4.1} & 53.4$\pm$\small{3.8} & 41.5$\pm$\small{2.7} & 52.7$\pm$\small{1.5} & 41.4$\pm$\small{2.8} \\
  Hazelnut & 37.6$\pm$\small{0.0} & 45.4$\pm$\small{0.0} & 68.9$\pm$\small{2.6} & 72.7$\pm$\small{3.7} & 70.5$\pm$\small{1.7} & 74.2$\pm$\small{3.8} & 71.0$\pm$\small{0.3} & 76.0$\pm$\small{1.1} \\
   Leather & 39.7$\pm$\small{0.0} & 50.2$\pm$\small{0.0} & 58.0$\pm$\small{0.7} & 59.9$\pm$\small{2.3} & 57.5$\pm$\small{0.6} & 58.9$\pm$\small{1.7} & 56.3$\pm$\small{1.0} & 57.3$\pm$\small{1.5} \\
 Metal nut & 32.4$\pm$\small{0.0} & 30.1$\pm$\small{0.0} & 59.4$\pm$\small{1.7} & 61.5$\pm$\small{2.2} & 62.7$\pm$\small{1.5} & 64.1$\pm$\small{3.1} & 67.4$\pm$\small{1.6} & 68.4$\pm$\small{3.4} \\
      Pill & 17.6$\pm$\small{0.0} & 21.3$\pm$\small{0.0} & 64.7$\pm$\small{1.8} & 64.0$\pm$\small{1.7} & 67.8$\pm$\small{0.5} & 65.9$\pm$\small{0.8} & 67.9$\pm$\small{0.4} & 67.0$\pm$\small{0.8} \\
     Screw & 13.5$\pm$\small{0.0} & 25.8$\pm$\small{0.0} & 22.2$\pm$\small{2.8} & 16.7$\pm$\small{3.7} & 22.4$\pm$\small{2.8} & 19.5$\pm$\small{6.0} & 30.1$\pm$\small{4.3} & 19.0$\pm$\small{8.5} \\
      Tile & 32.6$\pm$\small{0.0} & 56.4$\pm$\small{0.0} & 71.2$\pm$\small{0.4} & 58.8$\pm$\small{1.2} & 71.9$\pm$\small{0.6} & 59.1$\pm$\small{1.1} & 72.2$\pm$\small{0.6} & 58.9$\pm$\small{0.8} \\
Toothbrush & 17.1$\pm$\small{0.0} & 23.2$\pm$\small{0.0} & 62.7$\pm$\small{3.6} & 63.5$\pm$\small{5.7} & 65.8$\pm$\small{2.2} & 63.6$\pm$\small{3.7} & 69.4$\pm$\small{4.6} & 66.2$\pm$\small{2.8} \\
Transistor & 30.5$\pm$\small{0.0} & 19.6$\pm$\small{0.0} & 39.1$\pm$\small{3.5} & 39.6$\pm$\small{2.7} & 45.6$\pm$\small{2.3} & 43.1$\pm$\small{1.4} & 46.6$\pm$\small{2.2} & 46.2$\pm$\small{1.3} \\
      Wood & 51.5$\pm$\small{0.0} & 67.2$\pm$\small{0.0} & 65.2$\pm$\small{1.4} & 63.9$\pm$\small{1.0} & 65.8$\pm$\small{0.6} & 63.7$\pm$\small{0.8} & 65.1$\pm$\small{0.5} & 63.4$\pm$\small{0.9} \\
    Zipper & 34.4$\pm$\small{0.0} & 46.5$\pm$\small{0.0} & 50.6$\pm$\small{3.9} & 53.0$\pm$\small{1.2} & 50.9$\pm$\small{4.5} & 51.8$\pm$\small{1.1} & 52.8$\pm$\small{2.7} & 52.0$\pm$\small{1.3} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & 31.7$\pm$\small{0.0} & \textbf{39.8$\pm$\small{0.0}} & \textbf{55.9$\pm$\small{2.7}} & 54.6$\pm$\small{1.1} & \textbf{58.4$\pm$\small{1.7}} & 55.8$\pm$\small{1.0} & \textbf{59.5$\pm$\small{1.8}} & 57.0$\pm$\small{0.8} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly segmentation (AS) performance in terms of class-wise $F_1$-max on MVTec-AD. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_as_mvtec_f1_max}
\end{table*}


==> tables/classlevel/as_mvtec_pauroc.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.73\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
MVTec-AD (AS) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    pAUROC &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Bottle & 89.5$\pm$\small{0.0} & 89.7$\pm$\small{0.0} & 97.5$\pm$\small{0.2} & 96.4$\pm$\small{0.3} & 97.7$\pm$\small{0.1} & 96.7$\pm$\small{0.2} & 97.8$\pm$\small{0.0} & 96.7$\pm$\small{0.3} \\
     Cable & 77.0$\pm$\small{0.0} & 80.1$\pm$\small{0.0} & 93.8$\pm$\small{0.6} & 94.0$\pm$\small{0.3} & 94.3$\pm$\small{0.4} & 94.4$\pm$\small{0.4} & 94.9$\pm$\small{0.1} & 94.8$\pm$\small{0.2} \\
   Capsule & 86.9$\pm$\small{0.0} & 89.5$\pm$\small{0.0} & 94.6$\pm$\small{0.8} & 97.0$\pm$\small{0.5} & 96.4$\pm$\small{0.3} & 97.6$\pm$\small{0.7} & 96.2$\pm$\small{0.5} & 98.2$\pm$\small{0.1} \\
    Carpet & 95.4$\pm$\small{0.0} & 99.3$\pm$\small{0.0} & 99.4$\pm$\small{0.0} & 99.4$\pm$\small{0.1} & 99.3$\pm$\small{0.0} & 99.4$\pm$\small{0.0} & 99.3$\pm$\small{0.0} & 99.4$\pm$\small{0.0} \\
      Grid & 82.2$\pm$\small{0.0} & 98.4$\pm$\small{0.0} & 96.8$\pm$\small{1.0} & 96.1$\pm$\small{1.1} & 97.7$\pm$\small{0.8} & 96.2$\pm$\small{0.7} & 98.0$\pm$\small{0.2} & 96.7$\pm$\small{0.7} \\
  Hazelnut & 94.3$\pm$\small{0.0} & 97.1$\pm$\small{0.0} & 98.5$\pm$\small{0.2} & 99.2$\pm$\small{0.2} & 98.7$\pm$\small{0.1} & 99.3$\pm$\small{0.2} & 98.8$\pm$\small{0.0} & 99.4$\pm$\small{0.1} \\
   Leather & 96.7$\pm$\small{0.0} & 99.2$\pm$\small{0.0} & 99.3$\pm$\small{0.0} & 99.4$\pm$\small{0.0} & 99.3$\pm$\small{0.0} & 99.4$\pm$\small{0.0} & 99.3$\pm$\small{0.0} & 99.4$\pm$\small{0.0} \\
 Metal nut & 61.0$\pm$\small{0.0} & 69.5$\pm$\small{0.0} & 90.0$\pm$\small{0.6} & 91.6$\pm$\small{0.6} & 91.4$\pm$\small{0.4} & 92.4$\pm$\small{0.9} & 92.9$\pm$\small{0.4} & 93.7$\pm$\small{1.0} \\
      Pill & 80.0$\pm$\small{0.0} & 84.4$\pm$\small{0.0} & 96.4$\pm$\small{0.3} & 96.2$\pm$\small{0.7} & 97.0$\pm$\small{0.2} & 96.7$\pm$\small{0.2} & 97.1$\pm$\small{0.0} & 96.8$\pm$\small{0.2} \\
     Screw & 89.6$\pm$\small{0.0} & 97.9$\pm$\small{0.0} & 94.5$\pm$\small{0.4} & 96.2$\pm$\small{0.8} & 95.2$\pm$\small{0.3} & 96.6$\pm$\small{1.0} & 96.0$\pm$\small{0.5} & 96.6$\pm$\small{1.0} \\
      Tile & 77.6$\pm$\small{0.0} & 92.7$\pm$\small{0.0} & 96.3$\pm$\small{0.2} & 93.7$\pm$\small{0.3} & 96.5$\pm$\small{0.1} & 93.9$\pm$\small{0.3} & 96.6$\pm$\small{0.1} & 93.8$\pm$\small{0.2} \\
Toothbrush & 86.9$\pm$\small{0.0} & 90.8$\pm$\small{0.0} & 97.8$\pm$\small{0.1} & 98.6$\pm$\small{0.3} & 98.1$\pm$\small{0.1} & 98.8$\pm$\small{0.2} & 98.4$\pm$\small{0.5} & 99.0$\pm$\small{0.1} \\
Transistor & 74.7$\pm$\small{0.0} & 62.8$\pm$\small{0.0} & 85.0$\pm$\small{1.8} & 82.8$\pm$\small{3.3} & 88.3$\pm$\small{1.0} & 85.7$\pm$\small{2.2} & 88.5$\pm$\small{1.2} & 88.5$\pm$\small{1.3} \\
      Wood & 93.4$\pm$\small{0.0} & 97.1$\pm$\small{0.0} & 94.6$\pm$\small{1.0} & 95.0$\pm$\small{0.8} & 95.3$\pm$\small{0.4} & 95.3$\pm$\small{0.3} & 95.4$\pm$\small{0.2} & 95.3$\pm$\small{0.2} \\
    Zipper & 91.6$\pm$\small{0.0} & 95.0$\pm$\small{0.0} & 93.9$\pm$\small{0.8} & 94.9$\pm$\small{0.5} & 94.1$\pm$\small{0.7} & 94.3$\pm$\small{0.2} & 94.2$\pm$\small{0.4} & 94.4$\pm$\small{0.1} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & 85.1$\pm$\small{0.0} & \textbf{89.6$\pm$\small{0.0}} & 95.2$\pm$\small{0.5} & \textbf{95.4$\pm$\small{0.3}} & \textbf{96.0$\pm$\small{0.3}} & 95.8$\pm$\small{0.2} & \textbf{96.2$\pm$\small{0.3}} & \textbf{96.2$\pm$\small{0.1}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly segmentation (AS) performance in terms of class-wise pixel-AUROC on MVTec-AD. We report the mean
and standard deviation over 5 random seeds.
}
\label{tab:classlevel_as_mvtec_pauroc}
\end{table*}


==> tables/classlevel/as_mvtec_pro.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.73\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
MVTec-AD (AS) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    PRO &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Bottle & 76.4$\pm$\small{0.0} & 80.3$\pm$\small{0.0} & 91.2$\pm$\small{0.4} & 89.1$\pm$\small{0.7} & 91.8$\pm$\small{0.3} & 89.2$\pm$\small{0.3} & 91.6$\pm$\small{0.2} & 89.3$\pm$\small{0.4} \\
     Cable & 42.9$\pm$\small{0.0} & 68.1$\pm$\small{0.0} & 72.5$\pm$\small{2.3} & 84.4$\pm$\small{0.4} & 74.7$\pm$\small{2.3} & 85.9$\pm$\small{0.4} & 77.0$\pm$\small{1.1} & 87.1$\pm$\small{0.4} \\
   Capsule & 62.1$\pm$\small{0.0} & 86.1$\pm$\small{0.0} & 85.6$\pm$\small{2.7} & 92.2$\pm$\small{1.4} & 90.6$\pm$\small{0.6} & 93.9$\pm$\small{2.1} & 90.1$\pm$\small{1.5} & 95.6$\pm$\small{0.2} \\
    Carpet & 84.1$\pm$\small{0.0} & 98.0$\pm$\small{0.0} & 97.4$\pm$\small{0.4} & 97.7$\pm$\small{0.2} & 97.3$\pm$\small{0.3} & 97.6$\pm$\small{0.3} & 97.0$\pm$\small{0.2} & 97.5$\pm$\small{0.1} \\
      Grid & 57.0$\pm$\small{0.0} & 94.8$\pm$\small{0.0} & 90.5$\pm$\small{2.7} & 89.7$\pm$\small{2.2} & 92.8$\pm$\small{2.5} & 89.8$\pm$\small{1.3} & 93.6$\pm$\small{0.6} & 90.7$\pm$\small{1.9} \\
  Hazelnut & 81.6$\pm$\small{0.0} & 92.6$\pm$\small{0.0} & 93.7$\pm$\small{0.9} & 94.4$\pm$\small{1.0} & 94.2$\pm$\small{0.3} & 95.0$\pm$\small{0.9} & 94.2$\pm$\small{0.3} & 95.5$\pm$\small{0.6} \\
   Leather & 91.1$\pm$\small{0.0} & 98.2$\pm$\small{0.0} & 98.6$\pm$\small{0.0} & 98.6$\pm$\small{0.3} & 98.3$\pm$\small{0.4} & 98.5$\pm$\small{0.2} & 98.0$\pm$\small{0.4} & 98.1$\pm$\small{0.3} \\
 Metal nut & 31.8$\pm$\small{0.0} & 69.2$\pm$\small{0.0} & 84.7$\pm$\small{1.1} & 87.3$\pm$\small{0.6} & 86.7$\pm$\small{0.8} & 88.1$\pm$\small{1.0} & 89.4$\pm$\small{0.1} & 89.7$\pm$\small{1.1} \\
      Pill & 65.0$\pm$\small{0.0} & 84.4$\pm$\small{0.0} & 93.5$\pm$\small{0.2} & 94.8$\pm$\small{0.3} & 94.5$\pm$\small{0.2} & 95.0$\pm$\small{0.2} & 94.6$\pm$\small{0.3} & 95.1$\pm$\small{0.1} \\
     Screw & 68.5$\pm$\small{0.0} & 91.5$\pm$\small{0.0} & 82.3$\pm$\small{1.1} & 85.7$\pm$\small{2.0} & 84.1$\pm$\small{0.5} & 87.5$\pm$\small{2.8} & 86.3$\pm$\small{1.8} & 87.5$\pm$\small{3.1} \\
      Tile & 51.2$\pm$\small{0.0} & 80.6$\pm$\small{0.0} & 89.4$\pm$\small{0.4} & 82.1$\pm$\small{1.0} & 89.6$\pm$\small{0.4} & 82.5$\pm$\small{0.6} & 89.9$\pm$\small{0.3} & 82.3$\pm$\small{0.6} \\
Toothbrush & 67.7$\pm$\small{0.0} & 89.7$\pm$\small{0.0} & 85.3$\pm$\small{1.0} & 86.8$\pm$\small{2.0} & 84.7$\pm$\small{1.4} & 88.6$\pm$\small{1.1} & 86.0$\pm$\small{3.3} & 89.7$\pm$\small{1.0} \\
Transistor & 43.4$\pm$\small{0.0} & 55.1$\pm$\small{0.0} & 65.0$\pm$\small{1.8} & 65.4$\pm$\small{2.7} & 68.6$\pm$\small{1.1} & 67.8$\pm$\small{1.4} & 69.0$\pm$\small{1.1} & 71.3$\pm$\small{1.4} \\
      Wood & 74.1$\pm$\small{0.0} & 91.7$\pm$\small{0.0} & 91.0$\pm$\small{0.6} & 88.4$\pm$\small{1.1} & 91.8$\pm$\small{0.6} & 87.6$\pm$\small{2.4} & 91.7$\pm$\small{0.3} & 86.1$\pm$\small{1.7} \\
    Zipper & 71.7$\pm$\small{0.0} & 87.5$\pm$\small{0.0} & 86.0$\pm$\small{1.7} & 87.7$\pm$\small{0.7} & 86.4$\pm$\small{1.6} & 86.4$\pm$\small{0.3} & 86.9$\pm$\small{0.7} & 86.6$\pm$\small{0.3} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & 64.6$\pm$\small{0.0} & \textbf{84.5$\pm$\small{0.0}} & 87.1$\pm$\small{1.2} & \textbf{88.3$\pm$\small{0.3}} & 88.4$\pm$\small{0.9} & \textbf{88.9$\pm$\small{0.2}} & 89.0$\pm$\small{0.8} & \textbf{89.5$\pm$\small{0.2}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly segmentation (AS) performance in terms of class-wise PRO on MVTec-AD. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_as_mvtec_pro}
\end{table*}

==> tables/classlevel/as_visa_f1_max.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
VisA (AS) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    $F_1$-max &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Candle & 22.5$\pm$\small{0.0} & 13.6$\pm$\small{0.0} & 42.7$\pm$\small{1.7} & 30.1$\pm$\small{1.2} &  42.2$\pm$\small{0.8} & 30.0$\pm$\small{1.3} &  43.0$\pm$\small{0.9} & 30.2$\pm$\small{1.0} \\
  Capsules &  9.2$\pm$\small{0.0} & 11.8$\pm$\small{0.0} & 58.2$\pm$\small{1.3} & 31.4$\pm$\small{0.9} &  57.0$\pm$\small{3.7} & 35.0$\pm$\small{2.3} &  59.8$\pm$\small{1.8} & 37.9$\pm$\small{2.3} \\
    Cashew & 13.2$\pm$\small{0.0} & 13.0$\pm$\small{0.0} & 59.5$\pm$\small{2.1} & 69.0$\pm$\small{2.4} &  60.5$\pm$\small{2.4} & 71.3$\pm$\small{1.6} &  62.3$\pm$\small{1.1} & 72.9$\pm$\small{1.3} \\
Chewinggum & 41.1$\pm$\small{0.0} & 45.9$\pm$\small{0.0} & 65.3$\pm$\small{0.5} & 65.9$\pm$\small{1.7} &  64.8$\pm$\small{0.9} & 65.1$\pm$\small{1.4} &  65.2$\pm$\small{0.2} & 63.2$\pm$\small{1.0} \\
     Fryum & 22.1$\pm$\small{0.0} & 32.2$\pm$\small{0.0} & 50.8$\pm$\small{1.8} & 49.7$\pm$\small{0.4} &  54.8$\pm$\small{1.7} & 50.4$\pm$\small{1.0} &  56.5$\pm$\small{0.6} & 52.0$\pm$\small{0.5} \\
 Macaroni1 &  7.0$\pm$\small{0.0} & 17.9$\pm$\small{0.0} & 34.1$\pm$\small{1.7} & 27.2$\pm$\small{1.5} &  33.2$\pm$\small{1.9} & 28.9$\pm$\small{1.4} &  33.8$\pm$\small{0.9} & 29.3$\pm$\small{1.5} \\
 Macaroni2 &  1.0$\pm$\small{0.0} & 15.3$\pm$\small{0.0} & 34.4$\pm$\small{3.0} &  6.9$\pm$\small{3.0} &  29.9$\pm$\small{3.4} &  7.0$\pm$\small{1.8} &  35.1$\pm$\small{2.5} & 11.7$\pm$\small{2.4} \\
      PCB1 &  2.4$\pm$\small{0.0} &  6.4$\pm$\small{0.0} & 25.9$\pm$\small{2.6} & 59.8$\pm$\small{3.6} & 34.6$\pm$\small{16.2} & 63.9$\pm$\small{6.4} & 50.9$\pm$\small{20.4} & 70.8$\pm$\small{6.8} \\
      PCB2 &  4.7$\pm$\small{0.0} &  2.8$\pm$\small{0.0} & 18.7$\pm$\small{1.5} & 38.5$\pm$\small{1.4} &  24.0$\pm$\small{1.1} & 41.6$\pm$\small{1.2} &  27.8$\pm$\small{1.9} & 43.7$\pm$\small{0.7} \\
      PCB3 & 10.3$\pm$\small{0.0} &  3.3$\pm$\small{0.0} & 31.2$\pm$\small{6.7} & 36.7$\pm$\small{2.1} &  37.1$\pm$\small{2.8} & 41.9$\pm$\small{1.9} &  42.5$\pm$\small{1.1} & 45.3$\pm$\small{0.8} \\
      PCB4 & 32.0$\pm$\small{0.0} &  7.6$\pm$\small{0.0} & 22.8$\pm$\small{2.9} & 30.9$\pm$\small{4.0} &  30.6$\pm$\small{2.4} & 35.6$\pm$\small{1.4} &  31.9$\pm$\small{3.0} & 36.6$\pm$\small{1.3} \\
Pipe fryum & 12.3$\pm$\small{0.0} & 30.2$\pm$\small{0.0} & 51.8$\pm$\small{2.0} & 61.5$\pm$\small{3.8} &  53.6$\pm$\small{2.6} & 62.1$\pm$\small{3.3} &  55.1$\pm$\small{1.1} & 62.7$\pm$\small{1.4} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & 14.8$\pm$\small{0.0} & \textbf{16.7$\pm$\small{0.0}} & 41.3$\pm$\small{2.3} & \textbf{42.3$\pm$\small{0.5}} &  43.5$\pm$\small{3.3} & \textbf{44.4$\pm$\small{0.9}} &  \textbf{47.0$\pm$\small{3.0}} & 46.4$\pm$\small{0.7} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly segmentation (AS) performance in terms of class-wise $F_1$-max on VisA. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_as_visa_f1_max}
\end{table*}


==> tables/classlevel/as_visa_pauroc.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
VisA (AS) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    pAUROC &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
Candle & 88.9$\pm$\small{0.0} & 93.0$\pm$\small{0.0} & 97.4$\pm$\small{0.2} & 98.4$\pm$\small{0.1} & 97.7$\pm$\small{0.1} & 98.5$\pm$\small{0.1} & 97.8$\pm$\small{0.2} & 98.5$\pm$\small{0.1} \\
  Capsules & 81.6$\pm$\small{0.0} & 80.8$\pm$\small{0.0} & 96.4$\pm$\small{0.6} & 95.4$\pm$\small{0.4} & 96.8$\pm$\small{0.3} & 96.0$\pm$\small{0.3} & 97.1$\pm$\small{0.2} & 96.3$\pm$\small{0.4} \\
    Cashew & 84.7$\pm$\small{0.0} & 89.2$\pm$\small{0.0} & 98.5$\pm$\small{0.2} & 99.0$\pm$\small{0.1} & 98.5$\pm$\small{0.1} & 99.0$\pm$\small{0.1} & 98.7$\pm$\small{0.0} & 99.0$\pm$\small{0.1} \\
Chewinggum & 93.3$\pm$\small{0.0} & 99.1$\pm$\small{0.0} & 98.6$\pm$\small{0.1} & 98.9$\pm$\small{0.0} & 98.6$\pm$\small{0.1} & 98.9$\pm$\small{0.0} & 98.5$\pm$\small{0.1} & 98.8$\pm$\small{0.0} \\
     Fryum & 88.5$\pm$\small{0.0} & 94.0$\pm$\small{0.0} & 96.4$\pm$\small{0.3} & 96.7$\pm$\small{0.2} & 97.0$\pm$\small{0.2} & 96.8$\pm$\small{0.2} & 97.1$\pm$\small{0.1} & 97.1$\pm$\small{0.2} \\
 Macaroni1 & 70.9$\pm$\small{0.0} & 98.4$\pm$\small{0.0} & 96.4$\pm$\small{0.6} & 98.8$\pm$\small{0.6} & 96.5$\pm$\small{0.7} & 99.3$\pm$\small{0.0} & 97.0$\pm$\small{0.2} & 99.3$\pm$\small{0.1} \\
 Macaroni2 & 59.3$\pm$\small{0.0} & 97.4$\pm$\small{0.0} & 96.8$\pm$\small{0.4} & 95.7$\pm$\small{1.4} & 96.8$\pm$\small{0.6} & 96.4$\pm$\small{0.9} & 97.3$\pm$\small{0.3} & 97.0$\pm$\small{0.5} \\
      PCB1 & 61.2$\pm$\small{0.0} & 85.7$\pm$\small{0.0} & 96.6$\pm$\small{0.6} & 98.9$\pm$\small{0.1} & 97.0$\pm$\small{0.9} & 98.9$\pm$\small{0.1} & 98.1$\pm$\small{0.9} & 99.1$\pm$\small{0.1} \\
      PCB2 & 71.6$\pm$\small{0.0} & 87.3$\pm$\small{0.0} & 93.0$\pm$\small{0.4} & 97.7$\pm$\small{0.3} & 93.9$\pm$\small{0.2} & 98.1$\pm$\small{0.1} & 94.6$\pm$\small{0.4} & 98.5$\pm$\small{0.1} \\
      PCB3 & 85.3$\pm$\small{0.0} & 87.4$\pm$\small{0.0} & 94.3$\pm$\small{0.3} & 95.6$\pm$\small{0.2} & 95.1$\pm$\small{0.2} & 96.4$\pm$\small{0.1} & 95.8$\pm$\small{0.1} & 97.0$\pm$\small{0.1} \\
      PCB4 & 94.4$\pm$\small{0.0} & 88.9$\pm$\small{0.0} & 94.0$\pm$\small{0.9} & 95.3$\pm$\small{1.1} & 95.6$\pm$\small{0.3} & 96.1$\pm$\small{0.6} & 96.1$\pm$\small{0.3} & 96.6$\pm$\small{0.3} \\
Pipe fryum & 75.4$\pm$\small{0.0} & 96.7$\pm$\small{0.0} & 98.3$\pm$\small{0.2} & 99.3$\pm$\small{0.2} & 98.5$\pm$\small{0.2} & 99.3$\pm$\small{0.1} & 98.7$\pm$\small{0.1} & 99.3$\pm$\small{0.1} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & 79.6$\pm$\small{0.0} & \textbf{91.5$\pm$\small{0.0}} & 96.4$\pm$\small{0.4} & \textbf{97.5$\pm$\small{0.1}} & 96.8$\pm$\small{0.3} & \textbf{97.8$\pm$\small{0.1}} & 97.2$\pm$\small{0.2} & \textbf{98.0$\pm$\small{0.0}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly segmentation (AS) performance in terms of class-wise pixel-AUROC on VisA. We report the mean
and standard deviation over 5 random seeds.
}
\label{tab:classlevel_as_visa_pauroc}
\end{table*}


==> tables/classlevel/as_visa_pro.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
VisA (AS) & \multicolumn{2}{c}{$K=0$} & \multicolumn{2}{c}{$K=1$}     & \multicolumn{2}{c}{$K=2$}     & \multicolumn{2}{c}{$K=4$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    PRO &       WinCLIP &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} &       WinCLIP+ &          \textbf{FADE} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
    Candle & 83.5$\pm$\small{0.0} & 93.5$\pm$\small{0.0} & 94.0$\pm$\small{0.4} & 97.0$\pm$\small{0.2} & 94.2$\pm$\small{0.2} & 97.1$\pm$\small{0.2} & 94.4$\pm$\small{0.2} & 97.2$\pm$\small{0.1} \\
  Capsules & 35.3$\pm$\small{0.0} & 42.7$\pm$\small{0.0} & 73.6$\pm$\small{3.5} & 80.8$\pm$\small{1.1} & 75.9$\pm$\small{1.9} & 82.1$\pm$\small{0.8} & 77.0$\pm$\small{1.4} & 82.3$\pm$\small{0.7} \\
    Cashew & 76.4$\pm$\small{0.0} & 89.3$\pm$\small{0.0} & 91.1$\pm$\small{0.8} & 90.1$\pm$\small{1.5} & 90.4$\pm$\small{0.6} & 89.5$\pm$\small{1.3} & 91.3$\pm$\small{0.9} & 86.7$\pm$\small{2.8} \\
Chewinggum & 70.4$\pm$\small{0.0} & 91.9$\pm$\small{0.0} & 91.0$\pm$\small{0.5} & 87.0$\pm$\small{0.5} & 90.9$\pm$\small{0.7} & 86.8$\pm$\small{0.3} & 91.0$\pm$\small{0.4} & 86.4$\pm$\small{0.5} \\
     Fryum & 77.4$\pm$\small{0.0} & 90.7$\pm$\small{0.0} & 89.1$\pm$\small{1.0} & 92.5$\pm$\small{0.5} & 89.3$\pm$\small{0.2} & 92.6$\pm$\small{0.6} & 89.7$\pm$\small{0.5} & 92.6$\pm$\small{0.2} \\
 Macaroni1 & 34.3$\pm$\small{0.0} & 91.6$\pm$\small{0.0} & 84.6$\pm$\small{2.3} & 92.7$\pm$\small{2.6} & 85.2$\pm$\small{1.4} & 94.4$\pm$\small{0.8} & 86.8$\pm$\small{0.8} & 94.6$\pm$\small{0.4} \\
 Macaroni2 & 21.4$\pm$\small{0.0} & 84.5$\pm$\small{0.0} & 89.3$\pm$\small{2.4} & 82.0$\pm$\small{5.2} & 88.6$\pm$\small{1.7} & 83.1$\pm$\small{2.1} & 90.5$\pm$\small{1.3} & 85.8$\pm$\small{2.4} \\
      PCB1 & 26.3$\pm$\small{0.0} & 70.2$\pm$\small{0.0} & 82.5$\pm$\small{6.0} & 90.5$\pm$\small{0.7} & 83.8$\pm$\small{5.0} & 90.2$\pm$\small{1.9} & 87.9$\pm$\small{2.1} & 88.9$\pm$\small{2.1} \\
      PCB2 & 37.2$\pm$\small{0.0} & 61.8$\pm$\small{0.0} & 73.6$\pm$\small{1.5} & 86.1$\pm$\small{1.5} & 76.2$\pm$\small{0.9} & 87.9$\pm$\small{0.5} & 78.0$\pm$\small{1.3} & 89.6$\pm$\small{0.4} \\
      PCB3 & 56.1$\pm$\small{0.0} & 72.9$\pm$\small{0.0} & 79.5$\pm$\small{2.5} & 87.0$\pm$\small{1.7} & 82.3$\pm$\small{1.8} & 88.9$\pm$\small{1.2} & 84.2$\pm$\small{1.0} & 89.7$\pm$\small{0.6} \\
      PCB4 & 80.4$\pm$\small{0.0} & 67.7$\pm$\small{0.0} & 76.6$\pm$\small{4.1} & 85.3$\pm$\small{5.7} & 81.7$\pm$\small{1.2} & 88.4$\pm$\small{3.2} & 84.2$\pm$\small{0.7} & 90.1$\pm$\small{1.3} \\
Pipe fryum & 82.3$\pm$\small{0.0} & 94.6$\pm$\small{0.0} & 96.1$\pm$\small{0.6} & 95.9$\pm$\small{0.9} & 96.2$\pm$\small{0.6} & 96.1$\pm$\small{0.5} & 96.6$\pm$\small{0.2} & 96.3$\pm$\small{0.4} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
      Mean & 56.8$\pm$\small{0.0} & \textbf{79.3$\pm$\small{0.0}} & 85.1$\pm$\small{2.1} & \textbf{88.9$\pm$\small{0.7}} & 86.2$\pm$\small{1.4} & \textbf{89.8$\pm$\small{0.4}} & 87.6$\pm$\small{0.9} & \textbf{90.0$\pm$\small{0.4}} \\
\bottomrule
\end{tabular}
}

\caption{
    Comparison of anomaly segmentation (AS) performance in terms of class-wise PRO on VisA. We report the mean and
standard deviation over 5 random seeds.
}
\label{tab:classlevel_as_visa_pro}
\end{table*}

==> tables/lang_vis_aggregation.tex <==
\begin{table}[t]
\begin{center}
% \resizebox{3cm}{!}{
\begin{tabular}{ccc}
\toprule
Task & Shot & Aggregation \\
\midrule
AC & 0-shot & $s^{lang}$  \\
\cmidrule(lr){2-3}
& k-shot & $s^{lang}+s^{vis,k}$  \\
\midrule
AS & 0-shot & $\boldsymbol{M}^{lang}+\boldsymbol{M}^{vis,0}$  \\
\cmidrule(lr){2-3}
& k-shot & $\boldsymbol{M}^{lang}+\boldsymbol{M}^{vis,k}$  \\
\bottomrule
\end{tabular}
% }
\end{center}
\caption{
Language and vision guidance aggregation under different settings.
}
\label{tab:lang_vis_aggregation}
\end{table}

==> tables/main_ac.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%

\begin{tabular}{clcccccc}
\toprule
\multicolumn{2}{l}{Anomaly Classification} & \multicolumn{3}{c}{MVTec-AD} & \multicolumn{3}{c}{VisA} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
Setup & Method & AUROC & AUPR & $F1$-max & AUROC & AUPR & $F1$-max\\
\midrule
0-shot & WinCLIP & \textbf{91.8$\pm$\small{0.0}} & \textbf{96.5$\pm$\small{0.0}} & \textbf{92.9$\pm$\small{0.0}} & \textbf{78.1$\pm$\small{0.0}} & \textbf{81.2$\pm$\small{0.0}} & \textbf{79.0$\pm$\small{0.0}} \\
\cmidrule(lr){2-8}
& FADE (ours) & 90.0$\pm$\small{0.0} & 95.6$\pm$\small{0.0} & 92.4$\pm$\small{0.0} & 75.6$\pm$\small{0.0} & 78.5$\pm$\small{0.0} & 78.6$\pm$\small{0.0} \\
\midrule
1-shot & PatchCore & 83.4$\pm$\small{3.0} & 92.2$\pm$\small{1.5} & 90.5$\pm$\small{1.5} & 79.9$\pm$\small{2.9} & 82.8$\pm$\small{2.3} & 81.7$\pm$\small{1.6} \\
& WinCLIP+ & 93.1$\pm$\small{2.0} & 96.5$\pm$\small{0.9} & 93.7$\pm$\small{1.1} & 83.8$\pm$\small{4.0} & 85.1$\pm$\small{4.0} & 83.1$\pm$\small{1.7} \\
\cmidrule(lr){2-8}
& FADE (ours) & \textbf{93.9$\pm$\small{0.7}} & \textbf{96.8$\pm$\small{0.3}} & \textbf{94.8$\pm$\small{0.2}} & \textbf{86.7$\pm$\small{2.0}} & \textbf{87.9$\pm$\small{1.5}} & \textbf{84.7$\pm$\small{0.8}} \\
\midrule
2-shot & PatchCore & 86.3$\pm$\small{3.3} & 93.8$\pm$\small{1.7} & 92.0$\pm$\small{1.5} & 81.6$\pm$\small{4.0} & 84.8$\pm$\small{3.2} & 82.5$\pm$\small{1.8} \\
& WinCLIP+ & 94.4$\pm$\small{1.3} & 97.0$\pm$\small{0.7} & 94.4$\pm$\small{0.8} & 84.6$\pm$\small{2.4} & 85.8$\pm$\small{2.7} & 83.0$\pm$\small{1.4} \\
\cmidrule(lr){2-8}
& FADE (ours) & \textbf{95.2$\pm$\small{1.0}} & \textbf{97.6$\pm$\small{0.5}} & \textbf{95.0$\pm$\small{0.4}} & \textbf{89.2$\pm$\small{0.4}} & \textbf{90.2$\pm$\small{0.2}} & \textbf{85.9$\pm$\small{0.6}} \\
\midrule
4-shot & PatchCore & 88.8$\pm$\small{2.6} & 94.5$\pm$\small{1.5} & 92.6$\pm$\small{1.6} & 85.3$\pm$\small{2.1} & 87.5$\pm$\small{2.1} & 84.3$\pm$\small{1.3} \\
& WinCLIP+ & 95.2$\pm$\small{1.3} & 97.3$\pm$\small{0.6} & 94.7$\pm$\small{0.8} & 87.3$\pm$\small{1.8} & 88.8$\pm$\small{1.8} & 84.2$\pm$\small[1.6] \\
\cmidrule(lr){2-8}
& FADE (ours) & \textbf{96.3$\pm$\small{0.4}} & \textbf{98.1$\pm$\small{0.2}} & \textbf{95.5$\pm$\small{0.4}} & \textbf{90.7$\pm$\small{0.3}} & \textbf{91.9$\pm$\small{0.4}} & \textbf{87.0$\pm$\small{0.2}} \\
\bottomrule
\end{tabular}

}
\caption{
Comparison of AC performance on MVTec-AD and VisA. We report the mean and standard deviation over 5 random seeds. Bold indicates the best performance.
}
\label{tab:main_ac}
\end{table*}

==> tables/main_as.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%

\begin{tabular}{clcccccc}
\toprule
\multicolumn{2}{l}{Anomaly Segmentation} & \multicolumn{3}{c}{MVTec-AD} & \multicolumn{3}{c}{VisA} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
Setup & Method & pAUROC & PRO & $F1$-max & pAUROC & PRO & $F1$-max\\
\midrule
0-shot & WinCLIP & 85.1$\pm$\small{0.0} & 64.6$\pm$\small{0.0} & 31.7$\pm$\small{0.0} & 79.6$\pm$\small{0.0} & 56.8$\pm$\small{0.0} & 14.8$\pm$\small{0.0} \\
\cmidrule(lr){2-8}
& FADE (ours) & \textbf{89.6$\pm$\small{0.0}} & \textbf{84.5$\pm$\small{0.0}} & \textbf{39.8$\pm$\small{0.0}} & \textbf{91.5$\pm$\small{0.0}} & \textbf{79.3$\pm$\small{0.0}} & \textbf{16.7$\pm$\small{0.0}} \\
\midrule
1-shot & PatchCore & 92.0$\pm$\small{1.0} & 79.7$\pm$\small{2.0} & 50.4$\pm$\small{2.1} & 95.4$\pm$\small{0.6} & 80.5$\pm$\small{2.5} & 38.0$\pm$\small{1.9} \\
& WinCLIP+ & 95.2$\pm$\small{0.5} & 87.1$\pm$\small{1.2} & \textbf{55.9$\pm$\small{2.7}} & 96.4$\pm$\small{0.4} & 85.1$\pm$\small{2.1} & 41.3$\pm$\small{2.3} \\
\cmidrule(lr){2-8}
& FADE (ours) & \textbf{95.4$\pm$\small{0.3}} & \textbf{88.3$\pm$\small{0.3}} & 54.6$\pm$\small{1.1} & \textbf{97.5$\pm$\small{0.1}} & \textbf{88.9$\pm$\small{0.7}} & \textbf{42.3$\pm$\small{0.5}} \\
\midrule
2-shot & PatchCore & 93.3$\pm$\small{0.6} & 82.3$\pm$\small{1.3} & 53.0$\pm$\small{1.7} & 96.1$\pm$\small{0.5} & 82.6$\pm$\small{2.3} & 41.0$\pm$\small{3.9} \\
& WinCLIP+ & \textbf{96.0$\pm$\small{0.3}} & 88.4$\pm$\small{0.9} & \textbf{58.4$\pm$\small{1.7}} & 96.8$\pm$\small{0.3} & 86.2$\pm$\small{1.4} & 43.5$\pm$\small{3.3} \\
\cmidrule(lr){2-8}
& FADE (ours) & 95.8$\pm$\small{0.2} & \textbf{88.9$\pm$\small{0.2}} & 55.8$\pm$\small{1.0} & \textbf{97.8$\pm$\small{0.1}} & \textbf{89.8$\pm$\small{0.4}} & \textbf{44.4$\pm$\small{0.9}} \\
\midrule
4-shot & PatchCore & 94.3$\pm$\small{0.5} & 84.3$\pm$\small{1.6} & 55.0$\pm$\small{1.9} & 96.8$\pm$\small{0.3} & 84.9$\pm$\small{1.4} & 43.9$\pm$\small{3.1} \\
& WinCLIP+ & \textbf{96.2$\pm$\small{0.3}} & 89.0$\pm$\small{0.8} & \textbf{59.5$\pm$\small{1.8}} & 97.2$\pm$\small{0.2} & 87.6$\pm$\small{0.9} & \textbf{47.0$\pm$\small{3.0}} \\
\cmidrule(lr){2-8}
& FADE (ours) & \textbf{96.2$\pm$\small{0.1}} & \textbf{89.5$\pm$\small{0.2}} & 57.0$\pm$\small{0.8} & \textbf{98.0$\pm$\small{0.0}} & \textbf{90.0$\pm$\small{0.4}} & 46.4$\pm$\small{0.7} \\
\bottomrule
\end{tabular}

}
\caption{
Comparison of AS performance on MVTec-AD and VisA. We report the mean and standard deviation over 5 random seeds. Bold indicates the best performance.
}
\label{tab:main_as}
\end{table*}

